Tracktention: Leveraging Point Tracking to Attend Videos Faster and Better

Temporal consistency is critical in video prediction to ensure that outputs are coherent and free of artifacts. Traditional methods, such as temporal attention and 3D convolution, may struggle with significant object motion and may not capture long-range temporal dependencies in dynamic scenes. To address this gap, we propose the Tracktention Layer, a novel architectural component that explicitly integrates motion information using point tracks, i.e., sequences of corresponding points across frames. By incorporating these motion cues, the Tracktention Layer enhances temporal alignment and effectively handles complex object motions, maintaining consistent feature representations over time. Our approach is computationally efficient and can be seamlessly integrated into existing models, such as Vision Transformers, with minimal modification. It can be used to upgrade image-only models to state-of-the-art video ones, sometimes outperforming models natively designed for video prediction. We demonstrate this on video depth prediction and video colorization, where models augmented with the Tracktention Layer exhibit significantly improved temporal consistency compared to baselines.

==> figs/fig_attn.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.95\linewidth]{figs/fig_attn.pdf}
\caption{The \textbf{Attentional Sampling} module attends image features in correspondence of each track, as shown by the attention maps below each frame.
}%
\label{fig:fig_attn}
\end{figure}


==> figs/fig_teaser.tex <==
\begin{figure}[ht]
\centering
\vspace{-1em}
\includegraphics[width=0.96\linewidth]{figs/fig_teaser.pdf}
\vspace{-1em}
\caption{The \textbf{\mname Layer uses using point tracks (red boxes) and temporal attention to maintain consistent features over time.
}%
\label{fig:teaser}
\vspace{-1em}
\end{figure}


==> figs/fig_teaser2.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.96\linewidth]{figs/fig_teaser2.pdf}
\vspace{-1em}
\caption{\textbf{Error Rate vs. Run Time, Scaled by Model Size:} Our method achieves low error rates with moderate run times and model size, enabled by the efficient \mname mechanism for processing video data. $^\dagger$Test dataset used in training.}%
\label{fig:teaserfig2}
\vspace{-1em}
\end{figure}

